Evaluating Language Models on Cross-Language Code Functional Equivalence

Background: Large Language Models (LLMs) have demonstrated strong performance across a variety of code-understanding tasks, leading many to believe that they can reason about program semantics. However, existing evaluations primarily focus on single-language settings or rely on synthetically generated code, raising concerns about whether current results reflect true semantic understanding. Aims: We investigate whether LLMs can accurately judge functional equivalence across different programming languages in human-written code, a setting that requires deeper reasoning beyond superficial similarity. Method: We introduce PolyHuman, a dataset of human-written programs in CPP, Java, and Python. Using this dataset, we evaluate intra- and inter-language equivalence detection across open-weight and proprietary LLMs, selecting GPT-o4-mini as a representative model to assess stability. We then manually analyze 81 cases of systematic disagreement in which models incorrectly judge functional equivalence, examining the code logic and the generated Chain-of-Thought reasoning. Finally, we categorize these failures and compare them across GPT-o4-mini, Claude-Opus-4.7, and Gemini-3-Flash to determine whether they reflect model-specific issues or broader limitations of state-of-the-art LLMs. Results: We identify a difficulty-dependent breakdown in equivalence judgment (harder problems make the model increasingly prone to misclassifying non-equivalent code as equivalent), a model-specific sensitivity to programming language for the best-performing model (particularly a more conservative behavior on Python), and a partial reliance on similarity-based cues. GPT-o4-mini also shows substantial run-to-run instability under identical settings, indicating inconsistent rather than absent capability. Conclusions: Current LLMs do not reliably capture functional equivalence within or across languages.

==> Sections/Acknowledge.tex <==
\section*{Acknowledgments}
This research was partially supported by FUNCAP (BP6-00241-00276.01.00/25), CNPq (201708/2025-6, 403304/2025-3, 404406/2023-8, 403719/2024-0), FAPESQ-PB (268/2025), CAPES, and Google Cloud Research Credits Program with the award GCP19980904.


==> table/table1.tex <==
\renewcommand{\arraystretch}{1.3} 
\begin{table*}[t]
\centering
\caption{Dataset Statistics Comparison}
\label{tab:dataset-stats}

\newcolumntype{P}[1]{>{\centering\arraybackslash}p{#1}}

\begin{tabular}{@{}l | l | cc c c c P{1.1cm} P{1.1cm} P{1.1cm} @{}} 
\toprule
\multirow{2}{*}{\textbf{Category}} & \multirow{2}{*}{\textbf{Metric}} & \multicolumn{2}{c}{\textbf{EquiBench}} & & \textbf{SeqCoBench} & & \multicolumn{3}{c}{\textbf{PolyHuman}} \\
\cmidrule{3-4} \cmidrule{6-6} \cmidrule{8-10}
& & OJ-A & OJ-V & & Test Portion & & \multicolumn{3}{c}{Each of Sub-tasks (12 in total)} \\ 
\midrule

Language & & Python & Python & & Python & & C++ & Java & Python \\ 

\multirow{2}{*}{Pairs} & Equal & 200 & 200 & & 1860 & & -- & 5035 & -- \\ 
& Not Equal & 200 & 200 & & 2555 $->$ 1860 & & -- & 5035 & -- \\ 

\multirow{3}{*}{Lines of Code} & Min & 3 & 2 & & 2 & & 1 & 1 & 1 \\ 
& Max & 3403 & 4087 & & 50 & & 1233 & 1423 & 1042 \\
& Avg. & 82 & 70 & & 7.79 & & 48.52 & 109.88 & 34.78 \\ 
\bottomrule
\end{tabular}

\renewcommand{\arraystretch}{1.0} 
\end{table*}




==> table/table3.tex <==
\begin{table*}[t]
\centering
\caption{Performance on language-level functional equivalence tasks (Part 2)}
\label{tab:functional_equivalence_part2}
\resizebox{\textwidth}{!}{
\begin{tabular}{l l c c c c c c c c}
\hline
Model & Method
& \makecell{CPP\_Pass1\\vs\\CPP\_Pass2}
& \makecell{JAVA\_Pass1\\vs\\JAVA\_Pass2}
& \makecell{PYTHON3\_Pass1\\vs\\PYTHON3\_Pass2}
& \makecell{CPP\_Pass1\\vs\\CPP\_Fail}
& \makecell{JAVA\_Pass1\\vs\\JAVA\_Fail}
& \makecell{PYTHON3\_Pass1\\vs\\PYTHON3\_Fail}
& \makecell{CPP\_Pass1\\vs\\JAVA\_Pass1}
& \makecell{JAVA\_Pass1\\vs\\PYTHON3\_Pass1}
& \makecell{PYTHON3\_Pass1\\vs\\CPP\_Pass1} \\
\hline

\multirow{2}{*}{O4-mini}
& Peer 
& -- & -- & -- & -- & -- & -- & -- & -- & -- \\
& Our  
& 0.84 & 0.83 & 0.68 & 0.79 & 0.88 & 0.92 & 0.81 & 0.73 & 0.73 \\
\hline

\multirow{2}{*}{Qwen-2.5-7B-Instruct-Turbo}
& Peer 
& -- & -- & -- & -- & -- & -- & -- & -- & -- \\
& Our  
& 0.51 & 0.69 & 0.52 & 0.65 & 0.47 & 0.64 & 0.76 & 0.59 & 0.59 \\
\hline

\multirow{2}{*}{Mistral}
& Peer 
& -- & -- & -- & -- & -- & -- & -- & -- & -- \\
& Our  
& 0.99 & 0.99 & 0.97 & 0.10 & 0.06 & 0.17 & 0.02 & 0.04 & 0.03 \\
\hline
\end{tabular}
}
\end{table*}


==> table/table4.tex <==
\begin{table}[ht]
\centering
\scriptsize
\caption{Spearman Similarity Analysis}
\label{tab:spearman-sorted}
%\resizebox{\columnwidth}{!}{%
\begin{tabular}{l rr c rr} 
\toprule
& \multicolumn{2}{c}{\textbf{EQ}} & & \multicolumn{2}{c}{\textbf{NEQ}} \\
\cmidrule{2-3} \cmidrule{5-6}
\textbf{Metric} & \textbf{Rho ($\rho$)} & \textbf{P-Value} & & \textbf{Rho ($\rho$)} & \textbf{P-Value} \\
\midrule
CodeBLEU         & 0.8667 & 0.0012 && 0.6970  & 0.0251 \\
UniXcoder        & 0.8424 & 0.0022 && 0.3333  & 0.3466 \\
BGE-Code         & 0.7818 & 0.0075 && 0.5636  & 0.0897 \\
Lexsim           & 0.6848 & 0.0289 && -0.5030 & 0.1383 \\
GraphCodeBERT    & 0.6485 & 0.0425 && 0.4545  & 0.1869 \\
CodeBERT         & 0.4788 & 0.1615 && 0.7576  & 0.0111 \\
\bottomrule
\end{tabular}%
%}
\end{table}

==> table/table8.tex <==

\newcommand{\rotcat}[1]{\rotatebox[origin=c]{90}{\parbox{2.4cm}{\centering\bfseries #1}}}

\begin{table*}[t]
\centering
\small
\caption{Taxonomy of LLM-judge failure modes in assessing code functional
equivalence, derived from manual analysis of misclassified cases.}
\label{tab:failure-taxonomy}
\begin{tabularx}{\textwidth}{@{}c l X X r@{}}
\toprule
\textbf{Group} & \textbf{Sub-category} & \textbf{Description} & \textbf{Example} & \textbf{\#} \\
\midrule

\multirow{12}{*}{\rotcat{(1) Reasoning Failures}}
& (1.1) Premise-Insufficient Correctness Argument
& The reasoning maps the code to a known algorithm, but the mapping step is wrong, and the LLM then argues from the incorrect premise (e.g., treating a \texttt{for}--\texttt{if} snippet as binary search).
&  % TODO: example
&  \\
\addlinespace[2pt]
& (1.2) Premature Abstraction
& The LLM concludes without a sufficiently detailed analysis; the reasoning stops above the level at which the actual differences become visible.
&  % TODO: example
&  \\
\addlinespace[2pt]
& \quad (1.2.1) Pattern-Matching Pseudo-Verification
& \emph{Shallow abstraction.} The conclusion is drawn from structural similarity alone (e.g., one snippet is DFS, the other BFS, so they ``must'' be equal) without semantic analysis.
&  % TODO: example
&  \\
\addlinespace[2pt]
& \quad (1.2.2) Implementation-Semantics Elision
& \emph{Deep abstraction.} Reasoning is correct at the algorithmic, semantic, and mathematical levels, but the LLM ignores language-specific implementation details.
&  % TODO: example
&  \\
\addlinespace[2pt]
& (1.3) Incomplete Execution Tracing
& The LLM reasons at the implementation level but traces execution incorrectly, misjudging the evolution of variables, state, or control flow.
&  % TODO: example
&  \\
\addlinespace[2pt]
& (1.4) Equivalence Standard Misapplication
& The LLM blurs \emph{functional} and \emph{semantic} equivalence, e.g., treating two snippets as equal merely because both pass an online judge.
&  % TODO: example
&  \\
\midrule

\multirow{6}{*}{\rotcat{(2) Knowledge Failures}}
& (2.1) Built-in Functions
& Misunderstandings about language built-ins, such as Java's \texttt{HashMap}, array indexing semantics, or the \texttt{sort} and \texttt{Math.*} functions across languages.
&  % TODO: example
&  \\
\addlinespace[2pt]
& (2.2) Independent-Operation Coupling Error
& The LLM is confused when independently executed operations carry implicit spatial or relational correspondences (e.g., the aligned indices of two separately sorted arrays).
&  % TODO: example
&  \\
\addlinespace[2pt]
& (2.3) Implicit Co-write
& Correctness depends on an invariant or synchronization relationship maintained across multiple modifications to the same state (e.g., a variable updated both inside and outside a loop or branch).
&  % TODO: example
&  \\
\midrule

\rotcat{(3) Data}
& (3.1) Problem Has More Than One Valid Solution
& Two snippets may produce different outputs yet both be valid, since the ground truth is derived from whether the code passes the judge.
&  % TODO: example
&  \\
\midrule

\rotcat{(4) Label}
& (4.1) Verdict--Reasoning Mismatch
& The final verdict and the accompanying reasoning contradict each other.
&  % TODO: example
&  \\
\midrule

\rotcat{(5) Correct}
& (5.1) Genuine Non-Equivalence Identified
& The LLM's judgment is actually correct: it finds a test case on which the snippets genuinely differ, or correctly recognizes a possible error (e.g., non-equivalence from hash collisions).
&  % TODO: example
&  \\

\bottomrule
\end{tabularx}
\end{table*}
